Causal Bandits with Unknown Graph Structure

In causal bandit problems, the action set consists of interventions on variables of a causal graph. Several researchers have recently studied such bandit problems and pointed out their practical applications. However, all existing works rely on a restrictive and impractical assumption that the learner is given full knowledge of the causal graph structure upfront. In this paper, we develop novel causal bandit algorithms without knowing the causal graph. Our algorithms work well for causal trees, causal forests and a general class of causal graphs. The regret guarantees of our algorithms greatly improve upon those of standard multi-armed bandit (MAB) algorithms under mild conditions. Lastly, we prove our mild conditions are necessary: without them one cannot do better than standard MAB algorithms.

==> causal_forest.tex <==
In this section, we focus on the setting where the underlying causal graph is a causal forest (see Definition~\ref{def:forest}) \ambuj{definition of a causal forest is not very clear. also it is important to point out that "causal forest" has another meaning in the ML literature: use of random forests for estimating causal treatment effects}.
Many widely used causal DAGs including trees and bipartite graphs are examples of causal forest~\citep{greenewald2019sample}. \ambuj{last sentence didn't make much sense to me. i think once the causal forest definition is clarified, hopefully it'll be easy to see why bipartite graphs are examples of causal forests}
Bipartite graph applications can range from biological networks, biomedical networks, biomolecular networks to epidemiological networks ~\citep{burgos2008two,kontou2016network,pavlopoulos2018bipartite}.
%For causal forest, We propose an efficient algorithm (Algorithm~\ref{algo:forest}) that achieves $\widetilde{O}(K\max\{\frac{1}{\Delta^2}, \frac{1}{\varepsilon^2}\}(d+C)(\log n)^2+\sqrt{KT})$\footnote{Here $\widetilde{O}(\cdot)$ ignores poly-log terms non-regarding to $n$.} regret, where $C$ denotes the number of chain components in $\mathcal{E}(D)$.

\ambuj{not sure why we need separate sections for the tree and forest case. seems to be a waste of space}

In previous section, we provide CN-UCB with improved regret bound for the causal tree setting. 
Generalizing CN-UCB to causal forest (Algorithm~\ref{algo:forest}) is straightforward. 
%It is well-known in the causal inference literature that the only directed edges appearing in an essential graph are those v-structures~\cite{pearl1995theory}.
%Thus, the essential graph of a causal forest does not contain undirected components with unshield colliders and the true causal graph for each component is simply 
We simply run stage 1 and stage 2 of CN-UCB for every chain component (tree structure) of the causal forest essential graph until stage 2 finds a reward generating variable. 
Then, a standard UCB can be applied on the reduced intervention set. 

We denote the set of chordal components of $\mathcal{E}(D)$ and the component that contains $X_R$ by $\text{CC}(\mathcal{E}(D))$ and $\mathcal{T}_R$, respectively.


\begin{algorithm}[tbp]
	\centering
	\caption{CN-UCB for Causal Forest}
	\begin{algorithmic}[1]
		\STATE \textbf{Input: }Essential graph $\mathcal{E}(D)$, $K, \varepsilon, \Delta, B, T_2$.
		\STATE Perform $\text{do}()$ for $B$ times, collect $R_1, \ldots, R_B$, $\hat{R}\leftarrow\frac{1}{B}\sum_{b=1}^B R_b$.
		\FOR{$\mathcal{T}_0$ in $\text{CC}(\mathcal{E}(D))$}
		\STATE \textbf{Stage 1:} Find a directed subtree that contains $X_R$: $\widetilde{\mathcal{T}}_0\leftarrow$ Find Sub-tree($\mathcal{T}_0, K, B, \varepsilon, \Delta, \hat{R}$).
		\IF{$\widetilde{\mathcal{T}}_0$ is not empty}
		\STATE \textbf{Stage 2:} Find the key node that generates the reward: $X_R\leftarrow$ Find Key Node($\widetilde{\mathcal{T}}_0, K, B, \Delta,\hat{R}$).
		\STATE \textbf{Stage 3: }Apply UCB algorithm on $\mathcal{A}_R = \{\text{do}(X_R = k)\mid k=1,\ldots,K\}$ for $T_2$ rounds.
		\ENDIF
		\ENDFOR
	\end{algorithmic}
\label{algo:forest}
\end{algorithm}

\begin{thm}[Regret Guarantee for Algorithm~\ref{algo:forest}]
	\label{thm:forest}
	Suppose we run Algorithm~\ref{algo:forest} with $T\gg 2KB(d+C)\log_2 n:=T_1$ and $T_2 = T-T_1$, where $B = O(\max\{\frac{1}{\Delta^2}, \frac{1}{\varepsilon^2}\}\log\left(\frac{nK}{\delta}\right))$
	%$B = \max\{\frac{32}{\Delta^2}\log\left(\frac{8nK}{\delta}\right), \frac{2}{\varepsilon^2}\log\left(\frac{8n^2K^2}{\delta}\right)\}$ 
	and $0<\delta<1$.
	Define $C$ as the number of chain components in $\mathcal{E}(D)$.
	Then under Assumptions~\ref{assump:causal},~\ref{assump:bdd} and~\ref{assump:reward_gap}, with probability at least $1-\delta$, we have
	\begin{align}
	R_T 
	%= O(KBd+\sqrt{KT\log T}) 
	= \widetilde{O}\left(K\max\{\frac{1}{\Delta^2}, \frac{1}{\varepsilon^2}\}(d+C)(\log n)^2+\sqrt{KT}\right),
	\end{align}
	where $\widetilde{O}$ ignores poly-log terms non-regarding to $n$ and $d:=\max_{\mathcal{T}_0\in\text{CC}(\mathcal{E}(D))}d_{\mathrm{max}}(\mathcal{T}_0)$.
\end{thm}


==> warmup.tex <==
We start with a simple case where the learner knows reward is only generated by the root. 
This problem can be resolved by a two-stage approach: 1) learn the directed tree structure and 2) perform interventions only on the root variable.
Due to the special structure of directed trees, the first step is equivalent to figuring out the root variable once the tree skeleton is available. 
We thus summarize the main steps for this task in Algorithm~\ref{algo:causal_tree}.
\begin{algorithm}[htbp]
	\caption{Causal Tree Bandit}
	\begin{algorithmic}[1]
		\STATE \textbf{Input: }Tree skeleton $\mathcal{T}_0$ obtained from observational data, $B, \varepsilon, T_2$.
		\STATE \textbf{Stage 1: }$X_R\leftarrow$ Find Root($\mathcal{T}_0, B, \varepsilon, T_2$)
		\STATE \textbf{Stage 2: }Apply UCB algorithm on $\mathcal{A}_R = \{\text{do}(X_R) = k\mid k\in[K]\}$ for $T_2$ rounds.
	\end{algorithmic}
	\label{algo:causal_tree}
\end{algorithm}
\begin{defini}[Central Node~\citep{greenewald2019sample}] \label{def:cnode}
	A central node $v_c$ of a tree $G$ with respect to a distribution $q$ over the nodes is one for which $\max_{j\in N_G(v_c)} q(B_G^{v_c:X_j})\leq 1/2$. At least one such $v_c$ is guaranteed to exist for any distribution $q$.
\end{defini}
From previous section we learn that the essential graph of the causal tree can be obtained from the infinite amount of observational data. 
%Furthermore, it is well-known that the only directed edges that appear in an essential graph are those v-structures~\cite{pearl1995theory}. 
There is no v-structure in a directed tree, so the essential graph is just the skeleton and we take it as the input in Algorithm~\ref{algo:causal_tree}.

We follow the idea of central node algorithm in \cite{greenewald2019sample} for the causal tree discovery step.
In stage 1 (Algorithm~\ref{algo:find_root}), we maintain a distribution $q(\cdot)$ over $\mathcal{X}$ that describes how likely each variable being the root. 
We initialize a uniform prior distribution $q_0(X_1) = \cdots = q_0(X_n) = 1/n$ as there is no preference on any node at the beginning.
At every step $t$, Algorithm~\ref{algo:find_root} identifies a central node $v_c(t)$ formally defined in Definition~\ref{def:cnode}. 
Intuitively, a central node $v_c(t)$ with respect to distribution $q$ partitions $\mathcal{X}$ into $v_c(t)$ itself and disconnected branches $B_G^{v_c(t):X_j}$ where $X_j\in N_G(v_c(t))$. 
A central node guarantees that the weight for every branch corresponding to $q$ is no larger than $1/2$ to maintain the balance among branches.
Once we intervene on the central node $v_c(t)$, we collect samples for the neighbors of $v_c(t)$.
Due to the special structure of trees, only one of the branches $B_G^{v_c:X_j}$ is towards the upstream direction for non-root $v_c(t)$. 
The variable $Y\in N_G(v_c(t))$ that induces the upstream direction branch cannot be affected by an intervention over $v_c(t)$, while $v_c(t)$ has direct causal effects on all the remaining variables in $N_G(v_c(t))$. 
By estimating the causal effects from $v_c(t)$ to all its neighbors, at least half of the variables can be eliminated from the candidate set for the root.
The posterior $q_{t+1}(X)$ will be set as zero if $X$ is not in the upstream direction for $v_c(t)$.
In the end of this procedure, it is guaranteed only one of the variable has non-zero posterior probability, and this variable can only be the root. 
In stage 2, we simply apply a UCB algorithm on the reduced intervention set. 

\begin{algorithm}[tbp]
	\caption{Find Root}
	\label{algo:find_root}
	\textbf{Input:} Tree skeleton $G_0$, $B, \varepsilon, T_2$.\\
	\textbf{Initialization: } $t \leftarrow 0$, $q_0(X)\leftarrow\frac{1}{n}, \forall X\in\mathcal{X}$.
	\begin{algorithmic}[1]
		\WHILE{more than one $q_t(X)$ are non-zeros}
		\STATE Identify central node $v_c(t)\leftarrow$ Finding a central node ($G_0, q_t(\cdot)$).
		%\STATE $q_{t+1}(X)\leftarrow 1, \forall X\in\mathcal{X}$.
		\FOR{$z\in [K]$}
		\STATE Perform $\text{do}(v_c(t)=z)$ for $B$ times. Collect samples $Y_1^z,\ldots,Y_B^z$ for $Y\in N_{G_0}(v_c(t))$.
		\FOR{$Y\in N_{G_0}(v_c(t))$}
		\STATE $\hat{P}(Y=y|\text{do}(v_c(t)=z)) \leftarrow \frac{1}{B}\sum_{b=1}^{B}\mathbb{1}_{\{Y_b^z=y\}}$, for $y\in \text{Dom}(Y)$.
		\IF{$|P(Y=y)-\hat{P}(Y=y|\text{do}(v_c(t)=z))|>\varepsilon/2$ for some $y\in D(Y)$}
		\STATE $q_{t+1}(X)\leftarrow0,\forall X\in B_{\mathcal{T}_0}^{v_c(t):Y}$.
		\ENDIF
		\ENDFOR
		\ENDFOR
		\STATE $t\leftarrow t+1$.
		\STATE Normalize $q_t$ as a proper distribution vector.
		\ENDWHILE
	\end{algorithmic}
	\textbf{Output:} $\argmax_X q_t(X)$ or the only $X$ such that $q_t(X) \neq 0$.
\end{algorithm}

We present the regret of our two-stage approach in Theorem~\ref{thm:causal_tree}.

\begin{thm}[Regret garantee for Algorithm~\ref{algo:causal_tree}]
	\label{thm:causal_tree}
	Define $T_1 = K\lceil\log_2n\rceil \frac{2}{\varepsilon^2}\log\left(\frac{2n^2K^2}{\delta}\right)$ and $B = \frac{2}{\varepsilon^2}\log\left(\frac{2n^2K^2}{\delta}\right)$.
	Denote the total iteration by $T$ such that $T\gg T_1$ and $T_2:= T-T_1$.
	The expected cumulative regret for Algorithm~\ref{algo:causal_tree} is:
	\begin{align}
	\mathbb{E}\left[R_T\right] = O\left(K\lceil\log_2n\rceil \frac{1}{\varepsilon^2}\log\left(n^2K^2 T\right)+\sqrt{KT\log T}\right) = \tilde{O}(\frac{K}{\varepsilon^2}+\sqrt{KT}). \label{equ:ETC_regret}
	\end{align}
\end{thm}


